Utilizing Synthetic Data in Supervised Learning for Robust 5-DoF Magnetic Marker Localization

Tracking passive magnetic markers plays a vital role in advancing healthcare and robotics, offering the potential to significantly improve the precision and efficiency of systems. This technology is key to developing smarter, more responsive tools and devices, such as enhanced surgical instruments, precise diagnostic tools, and robots with improved environmental interaction capabilities. However, traditionally, the tracking of magnetic markers is computationally expensive due to the requirement for iterative optimization procedures. Moreover, these methods depend on the magnetic dipole model for their optimization function, which can yield imprecise outcomes due to the model's significant inaccuracies when dealing with short distances between non-spherical magnet and sensor.Our paper introduces a novel approach that leverages neural networks to bypass these limitations, directly inferring the marker's position and orientation to accurately determine the magnet's 5 DoF in a single step without initial estimation. Although our method demands an extensive supervised training phase, we mitigate this by introducing a computationally more efficient method to generate synthetic, yet realistic data using Finite Element Methods simulations. The benefits of fast and accurate inference significantly outweigh the offline training preparation. In our evaluation, we use different cylindrical magnets, tracked with a square array of 16 sensors. We perform the sensors' reading and position inference on a portable, neural networks-oriented single-board computer, ensuring a compact setup. We benchmark our prototype against vision-based ground truth data, achieving a mean positional error of 4 mm and an orientation error of 8 degrees within a 0.2x0.2x0.15 m working volume. These results showcase our prototype's ability to balance accuracy and compactness effectively in tracking 5 DoF.

==> archive_03-1_simulation_point_wise.tex <==

%\subsubsection{Procedure}
%\begin{itemize}
    % \item[S1] % \textbf{Tracking via Neural Network is Initialization-Free.}
    %         We first compare the influence of initialization of the estimation on the results of the tracking.

    %         We sample the random points as in Section \ref{sec:training_nn} and generate corresponding magnetic flux densities with the magnetic dipole model at the locations of sensors.
    %         In this way, the characteristics of the synthetic signals agree with the internal physical model in the optimization method.

    %         Then a range of positional and orientation perturbations are performed on the sampled points as an initial guess in optimization.
    %         The stopping criteria in terms of numerical and gradient difference is set to be small, so the optimization mostly stops when reaching the maximal number of iterations allowed \TL{how long is this?} \MW{We experimented with a range of maximum allowed iterations to investigate the relations between the number of iterations and the corresponding tracking performance.}
    %         The MLPs do not require initial estimation of the position and orientation of the magnet. Therefore, we show the one-shot predictions made by MLPs based on identical signals used in the iterative method.

    % \item[S2] % \textbf{Neural Networks Trained on Different Datasets.}
    %         In the previous experiment, MLPs are trained on data generated with the magnetic dipole model.
    %         Empirically, neural networks are powerful enough to further model the irregularities brought by potentially non-spherical shapes of magnets.
    %         In this experiment, we compare the performances of neural networks trained with data generated by two methods, one via FEM-data and coordinate transformation as in Section \ref{sec:fem_sim} for cylindrical magnets, and another one being the approximate data computed via magnetic dipole model.
    %         We use $1000$ points per magnet for evaluation.
    %         The target positions and orientations are identical for all $6$ magnets, with magnetic signals generated differently based on the corresponding FEM data to mimic the situation in hands-on experiments. The shapes of magnets used in the simulation are identical to those we adopt in hands-on experiments in Section \ref{sec:opt_eval}.
%     \item[S3] % \textbf{Running Time.}
%     \TL{Extend a bit, especially the first paragraph can be more direct in terms of "why do we care"}
%     \MW{Theoretically, the prediction of MLPs involves a multitude of additions and multiplications. In this experiment, we aim to compare the running time of the predicting process of the MLPs with the time consumed in tens of gradient optimizations in the iterative method.}
%             Moreover, the prediction of MLP also involves the process of feature engineering in the input layer.
%             % At the same time, the optimization-based methods require computations of gradients with respect to the estimated locations for $n_{iter}$ times.
%             We run the experiment on a laptop with Intel CPU i7-7500U.
% \end{itemize}

%\subsubsection{Results} \label{sec:syn_results}

% \begin{figure}
%     \centering
%         \begin{subfigure}[b]{\columnwidth}
%         \includegraphics[width=\textwidth]{figures/opt_pos_init_evo_up.pdf}
%         \caption{}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{\columnwidth}
%         \includegraphics[width=\textwidth]{figures/opt_pos_init_evo_down.pdf}
%         \caption{}
%         \end{subfigure}
%     \caption[Control Variable Experiments: optimized results vs. iterations]{
%     Positional errors of the optimization method when tracking random points in simulation, plotted in boxplot.
%          \textup{(a)} Optimization process starts at a fixed distance of $80$ mm to the truth.
%          \textup{(b)} Optimization process starts at a fixed orientation difference of $45^{\circ}$ w.r.t. the truth.
%       \label{fig:evo_angle_perturb}}
% \end{figure}

% \begin{table}
%     \caption[]{Tracking Errors of Optimization Methods for Randomly Simulated Points after 50 Iterations}
%     \label{tab:sim_opt_stats}
%     \centering
%     \begin{tabular}{>{\raggedleft}p{0.9cm}>{\raggedleft}p{0.9cm}|>{\raggedleft}p{0.9cm} >{\raggedleft}p{0.9cm} >{\raggedleft}p{1.3cm} >{\raggedleft\arraybackslash}p{1.3cm}}
%     \hline
%     Initial $e_p$ in mm &
%     Initial $e_{\theta}$ in degrees &
%     $\ \mathtt{median}$ $e_p$ in mm &
%     $\mathtt{median}$ $e_{\theta}$ in degrees &
%     % $\ \ \ \ \ \mathtt{max}$ $e_p$ in mm &
%     % $\ \ \mathtt{max}$ $e_{\theta}$ in degrees \\
%     $\mathtt{3^{rd} quartile}$ $e_p$ in mm &
%     $\mathtt{3^{rd} quartile}$ $e_{\theta}$ in degrees \\
%     \hline
%      % 80& 10& 1.10& 2.55& 908.19& 86.75 \\
%      % 80& 30& 2.98& 7.62& 876.38& 112.64 \\
%      % 80& 90& 45.60& 89.88& 897.36& 167.32 \\
%      % 80& 180& 103.48& 179.98& 878.23& 180.00 \\
%      80& 10& 1.28& 3.40& 52.79& 10.00 \\
%      80& 30& 3.77& 8.30& 48.35& 29.97 \\
%      80& 90& 37.14& 88.01& 87.32& 90.00 \\
%      80& 180& 86.89& 179.90& 165.00& 179.99 \\
%     \hline
%     % 30& 45& 0.69& 1.38& 876.58& 110.16 \\
%     % 60& 45& 3.59& 8.43& 27266.45& 169.36 \\
%     % 90& 45& 7.49& 16.85& 900.89& 129.00 \\
%     % 120& 45& 10.73& 28.33& 869.08& 132.93\\
%     30& 45& 0.86& 2.04& 14.55& 43.84 \\
%     60& 45& 4.55& 10.44& 62.87& 44.96 \\
%     90& 45& 8.56& 21.28& 57.48& 45.00 \\
%     120& 45& 13.98& 42.56& 61.51& 45.02 \\
%     \hline
%     \end{tabular}
% \end{table}
%\begin{itemize}
%     \item[S1] \textbf{Tracking via Neural Network is Initialization-Free.}
%     For the optimization method, we show the dependence of tracking errors on the initialization of the magnet's position and orientation in Figure \ref{fig:evo_angle_perturb}.
%     $400$ points are generated randomly as the target for optimization.
%     The statistics of tracking results after $50$ iterations is shown in Table \ref{tab:sim_opt_stats} and  Figure \ref{fig:evo_angle_perturb}.

%     For comparison, we applied neural networks for tracking with synthetic data identical to that in Figure \ref{fig:evo_angle_perturb}.
%     Since our MLP only takes the magnetic flux densities as an input, our results are independent of the initialization, or more accurately, there is no initialization.
%     We show the results of deploying trained MLPs for tracking in Table \ref{tab:sim_mlp_stats} where we the selection of different numbers of sensors are as in Section \ref{sec:hardware}, Figure \ref{fig:sensor_loc}. \TL{We really need to introduce and talk about this in the procedure.} \MW{(already explained in section II 3) hardware.)}\par

%     For both experiments testing the dependence of tracking error on initialization, only the cases with most iterations (50) and with the best initialization ($80$ mm of initial positional error and $10^\circ$ of initial orientation error in group A, $30$ mm of initial positional error and $30^\circ$ of initial orientation error in group B) outperform the results tracked by MLP. However, the computational time of the optimization-based method mounts to $50$ times longer than the time consumed by predicting via MLP, as we will discuss in S3.\par

%     For the worst case in group A with the most erroneous initialization (deviation of $80$ mm in the initial position and $180^\circ$ in initial orientation) and least iterations ($10$), the median value of positional errors exceeds $200$ mm, which is more than twice of the initial positional error. For the cases in group B (initial orientation error of $45^\circ$), $10$ iterations are not enough to bring the tracked results closer to truth since the median values of positional errors in optimized results are still comparable to the deviation in initialization.\par
%\end{itemize}


% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figures/sensors_used.pdf}
% %     \caption[]{Selections of Sensors for Neural Network Inputs
% %       \label{fig:sensor_sel}}
% % \end{figure}

% \begin{table}
%     \caption[]{Tracking Errors of MLPs in Predicting Randomly Simulated Points \TL{Do we also have the data to make this 3rd quartiles?}\MW{I intended to show, with maximum values, that the results are well bounded with no outliers. Not sure if this explanation compensates the inconsistency of the two tables.}}
%     \label{tab:sim_mlp_stats}
%     \centering
%     \begin{tabular}{>{\raggedleft}m{33pt}|>{\raggedleft}m{35pt} >{\raggedleft}m{25pt} >{\raggedleft}m{35pt} >{\raggedleft\arraybackslash}m{35pt}}
%     \hline
%      Number of sensors & $\mathtt{median}\ e_p $ in mm & $\mathtt{max}\ e_p$ in mm &
%     $\mathtt{median}\ {e_{\theta}}$ in degrees & $\mathtt{max}\ e_{\theta}$ in degrees \\
%      \hline
%      4& 2.00& 12.23& 5.31& 20.45 \\
%      8& 1.59& 7.36& 4.44& 23.99 \\
%      12& 1.56& 6.41& 4.05& 19.19 \\
%      16& 1.41& 5.66& 3.43& 18.18 \\
%     \hline
%     % \multicolumn{5}{c}{
%     % \includegraphics[width=0.65\linewidth]{figures/sensors_used.pdf}
%     %
%     % }
%     \end{tabular}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/dipole_vs_fem_MLP_pointwise_2.pdf}\\
%     \caption[]{Comparison of Errors When Applying Neural Networks Trained with Different Datasets on FEM-Simulated Signals
%       \label{fig:dipole_vs_mlp_nn}}
% \end{figure}

% \begin{itemize}
%     \item[S2] \textbf{Neural Networks Trained on Different Datasets.} \label{sec:syn_shapes}
%     The performances of neural networks trained on different datasets are compared in Figure \ref{fig:dipole_vs_mlp_nn}, where the shapes of magnets are ordered from pole-shape to thin disc-shaped, getting closer to a spherical shape and then deviating from it.
%     We used a Shapiro-Wilk test \cite{SHAPIRO1965} to validate the normal distribution of our data and then applied a Student's T-Test \cite{Ttest} to test for significant differences between dipole- and FEM-data trained MLPs.
%     We see a significant difference in all cases of cylindrical magnets and no significant difference for the spherical magnet.
%     The p-values of the Student's T-Tests are, ordered as in the figure, $6.21^{-7}, 1.23^{-6}, 0.95, 6.64^{-30}, 1.98^{-59}, 2.38^{-142}$.
%     We see a greater difference in the median values of errors where the magnets are less spherical.
% \end{itemize}

% \begin{itemize}
%     \item[S3] \textbf{Running Time.} \label{sec:eva_syn_runtime} The optimization-based algorithm takes around $1$ ms for one iteration in our setup. Depending on the initialization, we need a multitude of $10$ iterations to achieve satisfying results. On the other hand, the inference done with an MLP, including the feature engineering process, takes $0.8$ ms on the same device.
% \end{itemize}


==> archive_3-1_eval_simulation.tex <==
\subsection{Simulation}
\label{sec:mlp_evaluate}
% \TL{move to evaluation.}

\subsubsection{Trajectory Generation}
We build a trajectory generator that mimics the statistical characteristics of the movement of a magnet.
A sample-interpolate method is adopted to generate random trajectories.
Firstly, a granularity $r=\frac{N_{total}}{n_{sample}}$ is set and $n_{sample}$ points are generated randomly in the simulation space.
The metric is the summed virtual distances between the $n_{sample}$ points to determine the number of points to interpolate between samples.
The granularity $r$ and the weight of orientation difference with respect to the positional difference in virtual distances are hyper-parameters and tuned so that the synthetic trajectory resembles the experimental motions statistically.\par

\subsubsection{Accuracy}
We firstly simulate a trajectory and the corresponding magnetic flux densities with a simulated spherical magnet (magnetic moment $\mathbf{M}=1.6875$ A$\cdot$m$^2$).
The simple physical model is used to avoid the errors brought by the incompatibility of the magnetic dipole model in optimization and the non-spherical shape of a magnet.
The errors of trajectories tracked by the MLP and optimization algorithms are plotted in Figure \ref{fig:traj_sim}.
Here, the optimization-based tracking with $10$ updates per round fails to converge most of the time.
The MLP can achieve comparable results to optimization-based tracking with $20$ updates per round.
Although optimization-based tracking outperforms the neural network if more updates per round are allowed, it suffers from possible convergence failure, which results in big temporal errors.
In contrast, the predictions made by neural networks show much more stability.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/dipole_opt_results_uniform_legend.pdf}
    \caption[]{Errors of tracked trajectories by $4$ tracking methods in simulation with signals generated via magnetic dipole model.
    	  \textup{(a)} The norm of the positional difference (in m) between the truth and the tracked trajectory.
		\textup{(b)} The angular difference (in degree) between the true orientation and the tracked orientation.
      \label{fig:traj_sim}}
\end{figure}

% TODO: a table comparing the statistical results?

\subsubsection{Magnet Shapes}
One last benefit of training a neural network for tracking is that the dataset for training can be tailored to magnets with specific shapes with FEM deployed.
Since it is technically hard to integrate shape information into the physical model in the optimization algorithm,
the results of optimization-based tracking are expected to be worse than an MLP for non-spherical magnets, especially when the magnet is close to the sensors.\par
Figure \ref{fig:fem_opti_mlp} shows the tracking errors of a neural network trained with the data generated specifically for a cylindrical magnet.
The optimization tracking methods based on the magnetic dipole model suffer from deviation more frequently than in Figure \ref{fig:traj_sim} because the magnetic dipole model is applied on a non-spherical magnet.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fem_opt_results_uniform_legend.pdf}\\
    \caption[]{Errors of tracked trajectories by $4$ tracking methods in simulation with signals generated using a cylindrical magnet (height $20$ mm, radius $5$ mm).
    	  \textup{(a)} The norm of the positional difference (in m) between the truth and the tracked trajectory.
			  \textup{(b)} The angular difference (in degree) between the true orientation and the tracked orientation.
      \label{fig:fem_opti_mlp}}
\end{figure}

\subsubsection{Computational Time}
% \TL{Dont present new advantages here, they need to be clear in the method section.}
Another advantage of the neural network model lies in the speed of tracking.
Given the signals from sensors, tracking is done in a single inference of the neural network, which involves feature engineering, additions, and multiplications in hidden layers. At the same time, the optimization-based models require computations of second-order gradients with respect to the estimated locations for $n_{iter}$ times.\par
For the experiments in this section, we run the optimization-based algorithm on a PC with an intel i9-10900K CPU and $32$ GB of RAM.
The running time comparison is shown in Figure \ref{sim:running_time}.
The optimization-based method takes $0.07$ second for $10$ iterations per round, not to mention yielding unsatisfactory results. The neural network is able to track within milliseconds.
With the neural network models, the tracking tasks can now be moved to energy-restricted devices confidently with a high interactive rate.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/running_time_boxplot.pdf}
    \caption[Boxplot of Running Time for $4$ Tracking Methods]{The running time of tracking one step in simulation.
      \label{sim:running_time}}
\end{figure}

\subsubsection{Feature Engineering}
% \TL{This is in simulation right?}
\label{subsec:feat_eng}
A control-variable experiment is performed to investigate the effectiveness of the feature engineering function in Section \ref{subsub:mlp} and the batch normalization block.
Figure \ref{fig:loss_evo_bn} shows that evenly distributing the features by feature engineering is the key for the network to converge.
Taking the cubic root of inputs without batch normalization is the best method that has the lowest testing loss.
Therefore, we adopt the feature engineering function $f(B) = \sqrt[3]{B}$ for all the neural networks in evaluation.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/loss_evo_feat_eng.pdf}
    \caption[Testing Loss Evolution of Networks with Batch Normalization and/or Feature Engineering]{The testing loss with the identical $10^6$ random inputs per epoch fed to train networks with different input manipulations.
      \label{fig:loss_evo_bn}}
\end{figure}


% \input{2-4_rnn}


==> error_analysis.tex <==
\section{Analysis of Errors in Real-World Experiments}
% % TODO: maybe only keeping the last one: asynchronous reading
\label{sec:error_analysis}
% With the data sheet of sensors MLX90393 \cite{mlx90393}, Gaussian noises are added on the theorectical clean readings in Section \ref{sec:err_stat} to investigate the impact of noise on the trackin results.
With the parameter settings in experiments, the sensors have an data conversion time of $25$ ms
and therefore is specified by the manual to have standard deviations $\sigma_{B_{x,y}} = 6.0\cdot 10^{-7}$ Tesla and $\sigma_{B_{z}} = 9.66\cdot 10^{-7}$ Tesla.\par
% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\linewidth]{figures/percentile_plot.pdf}
%     % \captionsetup{singlelinecheck=off}
%     \caption[Statistical Plot of Trajectories Predicted with Synthetic Perturbed Sensor Readings]{
%     Histogram and percentile plot of positional errors for trajectories predicted with synthetic perturbed sensor readings.
%     % \MW{if applied with optimization algorithm, this histogram and percentile plot might be used to show the instability of optimization-based tracking?}
%     \label{fig:err_power_stat}}
% \end{figure}
% Figure \ref{fig:err_power_stat} indicates that in Section \ref{sec:err_stat}, the prediction from experimental magnetic signals have a similar performance to those predicted with synthetic readings perturbed with $10$ to $20$ times of theoretical sensor noise.
The following subsections are attempts verify if the noise level in experiments agrees with the one on the sensor manual.

\subsection{Drift of Background Noise}
At the beginning of all the hands-on experiments, $100$ sample readings without magnet are collected and averaged to get $\mathbf{B}_{background}$, which is subtracted from the signals collected later and not changed till the end of the experiment.
When collecting data in experiment, we noticed that even though the sensor is fixed at one location,
the background noise does not stay steady within the limit of standard deviation specified in the datasheet.
Therefore, an experiment investigating the drifting of background noise is conducted.
The magnet moves around the sensors and then is moved away for $40$ times.
% The magnet moves roughly $3$ centimeters away from the sensor to ensure that the magnetic field sensed does not exceed the limit of the sensor.
Each time when the magnet is away, $100$ readings of background noise are collected and averaged. \par
The statistics of the $40$ averaged background noise are documented in Table \ref{tab:noise_evo_stat},
with the standard deviation of background noise on $x$ and $y$ axes $2$ to $3$ times greater than those in that specified in datasheet.
The drift of background noise, with higher standard deviation than specified in datasheet, leads to the inaccuracy of the sensor readings collected in experiments, where $\mathbf{B}_{sensor} = \mathbf{B}_{raw} - \mathbf{B}_{background}$.\par
The reason for such drifting effect is unclear. The sensors might not recover to the original state after sensing a strong magnetic field.
Other possible explanations include changing background electromagnetic noises, minor perturbations on the sensors' locations, or slight thermal drifts which is not considered in all the experiments (the temperature of surrouding environment is assumed to be constant $25^\circ$C). \par

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/noise_evo}
%     \caption[Evolvement of Background Noise in Intervals of Collecting Data]{
%     Evolvement of background noise in the intervals of collecting data, with $1$ standard deviation range.
%     \TL{You dont need the orange and green line here. They seem different trajectories.}
%       \label{fig:noise_evo}}
% \end{figure}

\begin{table}
    \caption[Statistics of Background Noise Collected in Intervals of Collecting Data]{Statistics of background noise in the intervals of collecting data.}
    \label{tab:noise_evo_stat}
    \centering
    \begin{tabular}{c|cc}
    \hline
     Axis & mean (Tesla) & std. (Tesla) \\
     \hline
    x & $-2.14 \cdot 10^{-5}$  & $-1.51 \cdot 10^{-6}$ \\
    y & $-1.05 \cdot 10^{-4}$  & $-1.99 \cdot 10^{-6}$ \\
    z & $-1.08 \cdot 10^{-4}$  & $-1.01 \cdot 10^{-6}$ \\
    \hline
    \end{tabular}
\end{table}

\subsection{Asynchronous Data Collection}
% \TL{I think we go into too much detail here.}
Another factor to explain for the inaccuracy in sensor readings lies in the fact that the sensors are read in sequence, not simultaneously.
% The time span of collecting $n=16$ sensor readings is depicted in Figure \ref{fig:time_diff}.
% According to the specification of sensors, the data $\mathbf{B}^i_{\tau}$ read out at sensor $i$ in round $\tau$ went through a conversion time $\mathbf{T}_{conv}$ before it is available. This reading is present for another $\mathbf{T}_{conv}$ before a new reading is converted.
% Since the sensors are initialized asynchronously, we assume the time a sensor starts converting is random.
% The maximum difference between the time $\mathbf{B}^i_{\tau}$ and $\mathbf{B}^{i+k}_{\tau}$ are converted is $\mathbf{T}_{conv} + \mathbf{T}_{interval}$ and the minimum difference is $\mathbf{T}_{interval} - \mathbf{T}_{conv}$.
The averaged time difference between reading sensor $i$ and sensor $i+k$ is:

% \begin{align*}
% {\mathbf{T}_{int\_avg}} &= \frac{1}{\mathbf{T}_{end}^i - \mathbf{T}_{start}^i} \cdot \frac{1}{\mathbf{T}_{end}^{i+k} - \mathbf{T}_{start}^{i+k}} \\
% &\cdot \int\limits_{{t_i} = \mathbf{T}_{start}^i}^{\mathbf{T}_{end}^i} {\int\limits_{{t_{i + k}} = \mathbf{T}_{start}^{i + k}}^{\mathbf{T}_{end}^{i + k}} {({t_{i + k}} - {t_i})d{t_i}d{t_{i + k}}} }  \\
% &= \frac{1}{{{\mathbf{T}_{conv}}^2}} \cdot \frac{{\mathbf{T}_{conv}^2}}{2}\big(2 \cdot \mathbf{T}_{interval}\big)\\
% &= \frac{k}{n-1}\cdot \mathbf{T}_{reading}
% \end{align*}
\begin{align*}
\mathbf{\bar{T}_{i, i+k}} = \frac{k}{n-1}\cdot \mathbf{T}_{reading}
\end{align*}
According to the statistics of position difference in trajectories, with a tracking frequency of $40$ Hz, the magnet on average moves $2.512$ mm away from the previous tracked step with an orientation change of $1.435^\circ$.
Considering positional difference only, the magnet moves at a speed of $\frac{2.512}{1/40} = 100.48$ mm/s.
Figure \ref{fig:nn_runtime} indicates that the duration for reading $16$ sensors $\mathbf{T}_{reading}$ is around $28$ ms.
Therefore, the average positional difference between detecting $\mathbf{B}_{\tau}^i$ and $\mathbf{B}_{\tau}^{i+k}$ is $100.48 \cdot \frac{k}{n-1} * \frac{28}{1000} \approx \frac{2.8k}{n-1}$ mm. \par

The aligned sensor readings $(B_1^x, B_1^y, B_1^z, \ldots, B_n^x, B_n^y, B_n^z)$ are fed into the neural network to predict for positions and locations.
However, as analyzed above, each $\mathbf{B}^i$ maybe collected at different time and corresponds to different locations and orientations of the magnet.
Such non-synchronized sensor readings add to the final prediction error.
A possible solution is to have an shared external bus to trigger the conversion of data for all the sensors simultaneously.

% TODO: a plot to show the connection of sensors to Jetson.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/asynch_reading.pdf}
%     \caption[Time Plot of Reading Sensors Sequentially]{
%     Time plot illustrating the maximum possible time difference between when $\mathbf{B}^i_{\tau}$ and $\mathbf{B}^{i+k}_{\tau}$ are detected.
%       \label{fig:time_diff}}
% \end{figure}

% \subsubsection{Other Factors for Inaccurate Sensor Readings}
% One fundamental source of mismatch between theoretical values and sensor readings is that the locations of sensors / magnet that are used to compute for theoretical values is erroneous.
% The locations of magnets in Chapter \ref{chp:calibration} from the calibrator, the one tracked by OptiTrack \ref{sec:optitrack} for evaluation and the one in experiment \ref{subsec:sensor_scaling} are not perfectly precise.
% Moreover, the sensors' locations, either computed from modelling specifications or optimized with calibrator/OptiTrack, are neither absolutely truthful.
% Therefore, the theoretical values mentioned in this chapter serve as a dependable reference rather than a standard. The errors in such theoretical values also contributes to the error in evaluation.\par

